A Study of Feasibility and Diversity of Web Audio Fingerprints

Prior measurement studies on browser fingerprinting have unfortunately largely excluded Web Audio API-based fingerprinting in their analysis. We address this issue by conducting the first systematic study of effectiveness of web audio fingerprinting mechanisms. We focus on studying the feasibility and diversity properties of web audio fingerprinting. Along with 3 known audio fingerprinting vectors, we designed and implemented 4 new audio fingerprint vectors that work by obtaining FFTs of waveforms generated via different methods. Our study analyzed audio fingerprints from 2093 web users and presents new insights into the nature of Web Audio fingerprints. First, we show that audio fingeprinting vectors, unlike other prior vectors, reveal an apparent fickleness with some users' browsers giving away differing fingerprints in repeated attempts. However, we show that it is possible to devise a graph-based analysis mechanism to collectively consider all the different fingerprints of users and thus craft a stable fingerprinting mechanism. Our analysis also shows that it is possible to do this in a timely fashion. Next, we investigate the diversity of audio fingerprints and compare this with prior techniques. Our results show that audio fingerprints are much less diverse than other vectors with only 95 distinct fingerprints among 2093 users. At the same time, further analysis shows that web audio fingerprinting can potentially bring considerable additive value (in terms of entropy) to existing fingerprinting mechanisms. We also show that our results contradict the current security and privacy recommendations provided by W3C regarding audio fingerprinting. Overall, our systematic study allows browser developers to gauge the degree of privacy invasion presented by audio fingerprinting thus helping them take a more informed stance when designing privacy protection features in the future.

==> app_fp_results.tex <==
\onecolumn
\section{Complete Measurement Results}
\begin{figure}[H]
    \centering
    \subfloat[\centering Dynamic Compressor]{{\includegraphics[scale=0.5]{Stability/DynamicCompressor.png}\label{fig:DynamicCompressorBar}}}%
    \qquad
    \subfloat[\centering Oscillator Node]{{\includegraphics[scale=0.5]{Stability/OscillatorNode.png}\label{fig:OscillatorNodeBar}}}%
    \qquad
    \subfloat[\centering Channel Merge Hybrid]{{\includegraphics[scale=0.5]{Stability/ChannelMergeHybrid.png}\label{fig:ChannelMergeBar}}}%
    \qquad
    \subfloat[\centering Hybrid]{{\includegraphics[scale=0.5]{Stability/Hybrid.png}\label{fig:HybridBar}}}%
    \qquad
    \subfloat[\centering Custom Signal Hybrid]{{\includegraphics[scale=0.5]{Stability/CustomSignalHybrid.png}\label{fig:CustomSignalBar}}}%
    \qquad
    \subfloat[\centering Amplitude Modulation Hybrid]{{\includegraphics[scale=0.5]{Stability/AmplitudeModulationHybrid.png}\label{fig:AmplitudeModulationBar}}}%
    \qquad
    \caption[{Bar graphs showing grouping of the number of fingerprints observed for a fingerprinting method cont.}]{Bar graphs showing grouping of the number of fingerprints observed for a fingerprinting method cont.}
    \label{fig:StabilityBarGraphsCont}%
\end{figure}
\begin{figure}[H]
    \ContinuedFloat
    \centering
    \subfloat[\centering Frequency Modulation Hybrid]{{\includegraphics[scale=0.5]{Stability/FrequencyModulationHybrid.png}\label{fig:FrequencyModulationBar}}}%
    \caption[{Bar graphs showing grouping of the number of fingerprints observed for a fingerprinting method}]{Bar graphs showing grouping of the number of fingerprints observed for a fingerprinting method}
    \label{fig:StabilityBarGraphs}%
\end{figure}

\begin{figure}[h]
    \centering
    \includegraphics[scale=0.3]{browsers_users/DynamicCompressor.png}
    \caption[{Browser/OS combination of distinct fingerprint group for DynamicCompressor}]{Browser/OS combination of distinct fingerprint group for DynamicCompressor}
    \label{fig:BrowserOSDC}
\end{figure}

\begin{figure}[h]
    \centering
    \includegraphics[scale=0.3]{browsers_users/OscillatorNode.png}
    \caption[{Browser/OS combination of distinct fingerprint group for OscillatorNode}]{Browser/OS combination of distinct fingerprint group for OscillatorNode}
    \label{fig:BrowserOSON}
\end{figure}

\begin{figure}[h]
    \centering
    \includegraphics[scale=0.3]{browsers_users/Hybrid.png}
    \caption[{Browser/OS combination of distinct fingerprint group for Hybrid }]{Browser/OS combination of distinct fingerprint group for Hybrid}
    \label{fig:BrowserOSH}
\end{figure}

\begin{figure}[h]
    \centering
    \includegraphics[scale=0.3]{browsers_users/CustomSignalHybrid.png}
    \caption[{Browser/OS combination of distinct fingerprint group for CustomSignalHybrid}]{Browser/OS combination of distinct fingerprint group for CustomSignalHybrid}
    \label{fig:BrowserOSCS}
\end{figure}

\begin{figure}[h]
    \centering
    \includegraphics[scale=0.3]{browsers_users/ChannelMergeHybrid.png}
    \caption[{Browser/OS combination of distinct fingerprint group for ChannelMergeHybrid}]{Browser/OS combination of distinct fingerprint group for ChannelMergeHybrid}
    \label{fig:BrowserOSCM}
\end{figure}

\begin{figure}[h]
    \centering
    \includegraphics[scale=0.3]{browsers_users/AmplitudeModulationHybrid.png}
    \caption[{Browser/OS combination of distinct fingerprint group for AmplitudeModulationHybrid}]{Browser/OS combination of distinct fingerprint group for AmplitudeModulationHybrid}
    \label{fig:BrowserOSAM}
\end{figure}

\begin{figure}[h]
    \centering
    \includegraphics[scale=0.3]{browsers_users/FrequencyModulationHybrid.png}
    \caption[{Browser/OS combination of distinct fingerprint group for FrequencyModulationHybrid}]{Browser/OS combination of distinct fingerprint group for FrequencyModulationHybrid}
    \label{fig:BrowserOSFM}
\end{figure}

\setlength{\arrayrulewidth}{1mm}
\setlength{\tabcolsep}{3pt}
\renewcommand{\arraystretch}{1}
\begin{table}[ht]
\centering
    \begin{tabular}{lcccc}
    \toprule
    {\bf Fingerprinting Methods} & {\bf Distinct}& {\bf Unique} & {\bf Entropy} & {\bf Normalized Entropy}\\
    \midrule
    Canvas & 352 & 224 & 6.109 & 0.554 \\ 
    \midrule
    Fonts & 690 & 555 & 7.146 & 0.648 \\ 
    \midrule
    UserAgent & 427 & 284 & 6.466 & 0.586 \\ 
    \midrule
    Canvas + Font & 1106 & 916 & 9.086 & 0.824 \\ 
    \midrule
    Canvas + Audio & 492 & 318 & 6.699 & 0.607 \\ 
    \midrule
    Canvas + Font + UA & 1640 & 1436 & 10.422 & 0.945 \\ 
    \midrule
    Canvas + Font + Audio & 1210 & 1010 & 9.351 & 0.848 \\ 
    \midrule
    Audio FP & 95 & 49 & 2.803 & 0.254 \\ 
    \midrule
    Canvas + Font + UA + Audio & 1680 & 1493 & 10.479 & 0.95 \\ 
    \midrule
    \end{tabular}
    \caption{combination of different fingerprinting vectors}
    \label{table:CombinationFingerprints}
\end{table}

\setlength{\arrayrulewidth}{1mm}
\setlength{\tabcolsep}{3pt}
\renewcommand{\arraystretch}{1}
\begin{table}[ht]
\centering
    \begin{tabular}{lcccc}
    \toprule
    {\bf Fingerprinting Methods} & {\bf Distinct}& {\bf Unique} & {\bf Entropy} & {\bf Normalized Entropy}\\
    \midrule
    Canvas & 146 & 90 & 5.66 & 0.627 \\ 
    \midrule
    Fonts & 227 & 188 & 6.412 & 0.71 \\ 
    \midrule
    UserAgent & 159 & 111 & 5.849 & 0.647 \\ 
    \midrule
    Canvas + Font & 344 & 289 & 7.913 & 0.876 \\ 
    \midrule
    Canvas + Audio & 191 & 130 & 6.106 & 0.676 \\ 
    \midrule
    Canvas + Font + UA & 457 & 416 & 8.707 & 0.964 \\ 
    \midrule
    Canvas + Font + Audio & 365 & 311 & 8.061 & 0.892 \\ 
    \midrule
    Audio FP & 49 & 22 & 2.799 & 0.31 \\ 
    \midrule
    Canvas + Font + UA + Audio & 463 & 425 & 8.737 & 0.967 \\ 
    \midrule
    \end{tabular}
    \caption{combination of different fingerprinting vectors for first split }
    \label{table:CombinationFingerprints1}
\end{table}

\setlength{\arrayrulewidth}{1mm}
\setlength{\tabcolsep}{3pt}
\renewcommand{\arraystretch}{1}
\begin{table}[ht]
\centering
    \begin{tabular}{lcccc}
    \toprule
    {\bf Fingerprinting Methods} & {\bf Distinct}& {\bf Unique} & {\bf Entropy} & {\bf Normalized Entropy}\\
    Canvas & 145 & 87 & 5.701 & 0.631 \\ 
    \midrule
    Fonts & 217 & 170 & 6.426 & 0.712 \\ 
    \midrule
    UserAgent & 171 & 114 & 6.04 & 0.669 \\ 
    \midrule
    Canvas + Font & 347 & 288 & 7.981 & 0.884 \\ 
    \midrule
    Canvas + Audio & 192 & 137 & 6.189 & 0.685 \\ 
    \midrule
    Canvas + Font + UA & 476 & 443 & 8.828 & 0.978 \\ 
    \midrule
    Canvas + Font + Audio & 372 & 315 & 8.174 & 0.905 \\ 
    \midrule
    Audio FP & 44 & 17 & 2.739 & 0.303 \\ 
    \midrule
    Canvas + Font + UA + Audio & 482 & 451 & 8.858 & 0.981 \\ 
    \midrule
    \midrule 
    \end{tabular}
    \caption{combination of different fingerprinting vectors for second split}
    \label{table:CombinationFingerprints2}
\end{table}

\setlength{\arrayrulewidth}{1mm}
\setlength{\tabcolsep}{3pt}
\renewcommand{\arraystretch}{1}
\begin{table}[ht]
\centering
    \begin{tabular}{lcccc}
    \toprule
    {\bf Fingerprinting Methods} & {\bf Distinct}& {\bf Unique} & {\bf Entropy} & {\bf Normalized Entropy}\\
    \midrule
    Canvas & 159 & 103 & 5.881 & 0.651 \\ 
    \midrule
    Fonts & 229 & 183 & 6.59 & 0.73 \\ 
    \midrule
    UserAgent & 169 & 118 & 6.06 & 0.671 \\ 
    \midrule
    Canvas + Font & 360 & 307 & 8.035 & 0.89 \\ 
    \midrule
    Canvas + Audio & 213 & 157 & 6.41 & 0.71 \\ 
    \midrule
    Canvas + Font + UA & 474 & 441 & 8.808 & 0.975 \\ 
    \midrule
    Canvas + Font + Audio & 389 & 342 & 8.227 & 0.911 \\ 
    \midrule
    Audio FP & 47 & 27 & 2.809 & 0.311 \\ 
    \midrule
    Canvas + Font + UA + Audio & 477 & 444 & 8.828 & 0.978 \\ 
    \midrule
    \end{tabular}
    \caption{combination of different fingerprinting vectors for third split}
    \label{table:CombinationFingerprints3}
\end{table}

\setlength{\arrayrulewidth}{1mm}
\setlength{\tabcolsep}{3pt}
\renewcommand{\arraystretch}{1}
\begin{table}[ht]
\centering
    \begin{tabular}{lcccc}
    \toprule
    {\bf Fingerprinting Methods} & {\bf Distinct}& {\bf Unique} & {\bf Entropy} & {\bf Normalized Entropy}\\
    \midrule
    Canvas & 149 & 96 & 5.763 & 0.638 \\ 
    \midrule
    Fonts & 223 & 183 & 6.407 & 0.709 \\ 
    \midrule
    UserAgent & 183 & 126 & 6.148 & 0.681 \\ 
    \midrule
    Canvas + Font & 349 & 288 & 7.994 & 0.885 \\ 
    \midrule
    Canvas + Audio & 196 & 134 & 6.233 & 0.69 \\ 
    \midrule
    Canvas + Font + UA & 477 & 444 & 8.831 & 0.978 \\ 
    \midrule
    Canvas + Font + Audio & 378 & 322 & 8.194 & 0.907 \\ 
    \midrule
    Audio FP & 60 & 39 & 2.878 & 0.319 \\ 
    \midrule
    Canvas + Font + UA + Audio & 481 & 451 & 8.847 & 0.98 \\ 
    \midrule
    \end{tabular}
    \caption{combination of different fingerprinting vectors for fourth split }
    \label{table:CombinationFingerprints4}
\end{table}


\setlength{\arrayrulewidth}{1mm}
\setlength{\tabcolsep}{3pt}
\renewcommand{\arraystretch}{1}
\begin{table}[h]
\centering
    \begin{tabular}{lccc}
    \toprule
    {\bf Fingerprinting Methods} & {\bf Minimum} & {\bf Maximum} & {\bf Mean}\\
    \midrule
    DynamicCompressor & 1 & 1 & 1.0  \\ 
    \midrule
    OscillatorNode & 1 & 21 & 1.807  \\ 
    \midrule
    Hybrid & 1 & 18 & 2.082  \\ 
    \midrule
    CustomSignalHybrid & 1 & 18 & 2.084  \\ 
    \midrule
    ChannelMergeHybrid & 1 & 21 & 2.922  \\ 
    \midrule
    AmplitudeModulationHybrid & 1 & 26 & 4.284  \\ 
    \midrule
    FrequencyModulationHybrid & 1 & 24 & 4.334  \\ 
    \midrule
    \end{tabular}
    \caption{Number of users for each audio fingerprinting method}
    \label{table:time-analysis}
\end{table}

\setlength{\arrayrulewidth}{1mm}
\setlength{\tabcolsep}{3pt}
\renewcommand{\arraystretch}{1}
\begin{table}[ht]
\centering
    \begin{tabular}{lccccc}
    \toprule
    {\bf Fingerprinting Methods} & {\bf \# of Users}& {\bf Distinct}& {\bf Unique} & {\bf Entropy} & {\bf Normalized Entropy}\\
    \midrule
    Canvas & 2093 & 352 & 224 & 6.109 & 0.554 \\ 
    \midrule
    Fonts & 2093 & 690 & 555 & 7.146 & 0.648 \\ 
    \bottomrule
    DynamicCompressor & 2093 & 59 & 34 & 1.935 & 0.175 \\ 
    \midrule
    OscillatorNode & 2093 & 73 & 42 & 2.593 & 0.235 \\ 
    \midrule
    Hybrid & 2093 & 84 & 42 & 2.692 & 0.244 \\ 
    \midrule
    CustomSignalHybrid & 2093 & 72 & 41 & 2.582 & 0.234 \\ 
    \midrule
    ChannelMergeHybrid & 2093 & 87 & 45 & 2.767 & 0.251 \\ 
    \midrule
    AmplitudeModulationHybrid & 2093 & 82 & 45 & 2.69 & 0.244 \\ 
    \midrule
    FrequencyModulationHybrid & 2093 & 82 & 43 & 2.717 & 0.246 \\ 
    \midrule
    \end{tabular}
    \caption{Number of distinct and unique fingerprints and their entropy and normalized entropy }
\end{table}

\setlength{\arrayrulewidth}{1mm}
\setlength{\tabcolsep}{3pt}
\renewcommand{\arraystretch}{1}
\begin{table}[ht]
\centering
    \begin{tabular}{lccc}
    \toprule
    {\bf Fingerprinting Methods} & {\bf s-15}& {\bf s-10}& {\bf s-3} \\
    \midrule
    DynamicCompressor & 1.0 & 1.0 & 1.0 \\ 
    \midrule
    OscillatorNode & 1.0 & 1.0 & 0.9942 \\ 
    \midrule
    Hybrid & 1.0 & 1.0 & 0.9952 \\ 
    \midrule
    CustomSignalHybrid & 0.999 & 0.9988 & 0.9969 \\ 
    \midrule
    ChannelMergeHybrid & 1.0 & 0.9998 & 0.9953 \\ 
    \midrule
    AmplitudeModulationHybrid & 0.999 & 0.9983 & 0.991 \\ 
    \midrule
    FrequencyModulationHybrid & 0.9981 & 0.9978 & 0.9899 \\ 
    \midrule
    \end{tabular}
    \caption{Stability Score based on number of groups}
    \label{table:StabilityScore}
\end{table}

\begin{table}[H]
    \centering
        \begin{tabular}{lc}
        \toprule
        {\bf Fingerprinting Methods} & {\bf  \# of UAs spanning $>$ 1 FP goups }\\
        \midrule
        DynamicCompressor & 32 \\
        \midrule
        OscillatorNode & 89 \\
        \midrule
        Hybrid & 90 \\
        \midrule
        CustomSignalHybrid & 89 \\
        \midrule
        ChannelMergeHybrid & 90 \\
        \midrule
        AmplitudeModulationHybrid & 90 \\
        \midrule
        FrequencyModulationHybrid & 90 \\
        \midrule
        \end{tabular}
        \caption{Number of User-Agents spanning on more than 1 diverse fingerprint group}
        \label{table:useragentcomparision}
    \end{table}

==> fp_schematics.tex <==
\section{Fingerprinting Vector Schematics}
\subsection{DynamicCompressor Method}
\begin{figure}[H]
    \centering
    \includegraphics[width=1.0\columnwidth]{Schematics/DC.pdf}
    \caption[DynamicCompressor Full Buffer Method]{DynamicCompressor Full Buffer Method}
    \label{fig:DynamicCompressor}
\end{figure}

Figure~\ref{fig:DynamicCompressor}. shows the utilization of the \texttt{OfflineAudioContext}
interface to audio fingerprint the sound stack of a device. Initially, a triangle wave is
produced as shown in Figure \ref{fig:GeneratedTriangleWave} utilizing an \texttt{OscillatorNode}.
The signal is then connected to \texttt{DynamicsCompressorNode}, to increment differences in processed 
audio between devices. The yield of this compressor is passed to the buﬀer of an \texttt{OfflineAudioContext}.
Hashes generated from the values from the full buffer is used to audio fingerprint a user. This method was
found wild in the web by trackers during their 1-Million-Site Measurement and Analysis \cite{StevenEngleHardt}. 

\begin{figure}[H]
    \centering
    \includegraphics[scale=0.5]{WaveForms/TriangleGenerated.png}
    \caption[Generated Triangle Wave]{Generated Triangle Wave}
    \label{fig:GeneratedTriangleWave}
\end{figure}

\subsection{OscillatorNode Method}
\begin{figure}{h}
    \centering
    \includegraphics[scale=0.7]{Schematics/FFT.pdf}
    \caption[OscillatorNode Method]{OscillatorNode Method}
    \label{fig:OscillatorNode}
\end{figure}

Figure~\ref{fig:OscillatorNode}. shows the utilization of the \texttt{AudioContext} interface
to audio fingerprint the sound stack of a device. Initially, a triangle wave is created  as
shown in Figure \ref{fig:GeneratedTriangleWave} using an \texttt{OscillatorNode}.
This signal is then passed to an \texttt{AnalyserNode} and a \texttt{ScriptProcessorNode}.
At last, the single goes through a \texttt{GainNode} whose gain is set zero to mute any output to
\texttt{AudioContext} destination (For example. computer speakers). The \texttt{AnalyserNode} gives
admittance to a Fast Fourier Transform (FFT) of the audio signal, which is caught utilizing
the \emph{onaudioprocess} event handler added by the \texttt{ScriptProcessorNode}. 
The subsequent FFT is taken care of into a hash and utilized as a unique audio fingerprint.

\subsection{Hybrid Method}
\begin{figure}{h}
    \centering
    \includegraphics[width=1.0\columnwidth]{Schematics/Hybrid.pdf}
    \caption[{Hybrid (DynamicCompressor + OscillatorNode) Method}]{Hybrid (DynamicCompressor + OscillatorNode) Method}
    \label{fig:Hybrid}
\end{figure}

Figure~\ref{fig:Hybrid}. shows the combination of \texttt{OscillatorNode} and \texttt{DynamicCompressor}
methods to generate a unique audio fingerprint of a user using  \texttt{AudioContext} interface.
A triangle wave is generated as shown in Figure \ref{fig:GeneratedTriangleWave} using \\ \texttt{OscillatorNode}
which is passed through the \\ \texttt{DynamicsCompressorNode}. This signal is then passed to an
\texttt{AnalyserNode} and a \texttt{ScriptProcessorNode}. Similar to the \texttt{OscillatorNode} method the
signal then goes through \texttt{GainNode} that is set to zero. We use \texttt{AnalyserNode} to FFT the audio
signal, that is captured by \emph{onaudioprocess} event handler added by the \texttt{ScriptProcessorNode}.
The FFT is then hashed using MD5 which acts as an audio fingerprint.

\subsection{Custom Signal Hybrid Method}
\begin{figure}[h]
    \centering
    \includegraphics[scale=0.5]{Schematics/CustomSignal.jpg}
    \caption[{Custom Signal Hybrid Method}]{Custom Signal Hybrid Method}
    \label{fig:CustomSignalHybrid}
\end{figure}

Custom Signal Hybrid Method only differs from Hybrid method in terms of the signal.
Instead of using a standard signal (Sine, Triangle, Sawtooth, Square) offered by the
Web Audio API, we generate a periodic signal by defining the real and imaginary values
as shown in Appendix \ref{customSignalHybridFingerprintGenerationCode}.
Figure \ref{fig:CustomSignalHybrid}.
shows the setup used to generate a unique audio fingerprint of a user using  \texttt{AudioContext}
interface for custom signal. A custom periodic wave is generated as shown in Figure \ref{fig:GeneratedCustomWave}
using \texttt{AudioContext.createPeriodicWave()} method which is passed through the \texttt{DynamicsCompressorNode}.
This signal is then passed to an \texttt{AnalyserNode} and a \texttt{ScriptProcessorNode} as before.
Similar as before we use \texttt{AnalyserNode} to FFT audio signal, that is captured by \emph{onaudioprocess}
event handler added by the\\ \texttt{ScriptProcessorNode}. The FFT is then hashed using MD5 which acts as an
audio fingerprint.

\begin{figure}
    \centering
    \includegraphics[scale=0.5]{WaveForms/CustomWaveGenerated.png}
    \caption[Generated Custom Wave]{Generated Custom Wave}
    \label{fig:GeneratedCustomWave}
\end{figure}

\subsection{Audio Source Hybrid Method}
\begin{figure}[H]
    \centering
    \includegraphics[scale=0.6]{Schematics/AudioSource.jpg}
    \caption[{Audio Source Hybrid Method}]{Audio Source Hybrid Method}
    \label{fig:AudioSourceHybrid}
\end{figure}

Audio Source Hybrid is yet another new method that we introduced for audio fingerprinting. This method varies from all of the methods in terms of how the signal is generated.  In this method, we used a 40 seconds audio clip  \cite{AudioClip} that was trimmed down to 5 seconds to make it shorter and suitable for fingerprinting. The audio clip is first decoded using  \\ \texttt{AudioContext.decodeAudioData()} method to get the audio buffer which is then utilized by  \texttt{AudioContext.createBufferSource()} to generate the signal as shown in Figure \ref{fig:GeneratedAudioSourceWave}. This signal is then passed on to the rest of the audio nodes as before. Similarly, the \texttt{AnalyserNode} is used to FFT audio signal, that is captured by \emph{onaudioprocess} event handler added by the  \texttt{ScriptProcessorNode} and then hashed using MD5 to generate an audio fingerprint. Figure \ref{fig:AudioSourceHybrid} shows the method with different audio nodes used to generate an identifier.

\begin{figure}
    \centering
    \includegraphics[scale=0.075]{WaveForms/AudioSourceGenerated.png}
    \caption[Generated Audio Source Wave]{Generated Audio Source Wave}
    \label{fig:GeneratedAudioSourceWave}
\end{figure}

\subsection{Channel Merge Hybrid Method}
\begin{figure}
    \centering
    \includegraphics[width=1.0\columnwidth]{Schematics/Merged.pdf}
    \caption[{Channel Merge Hybrid Method}]{Channel Merge Hybrid Method}
    \label{fig:ChannelMergeHybrid}
\end{figure}

Channel Merge Hybrid is another addition to audio fingerprinting methods which was created during this research. The idea is to generate multiple signals and merge them using a \\ \texttt{ChannelMergeNode}. In this method we create four \texttt{OsciallatorNode} with different frequencies and different signal types and merge them together to generate a single waveform. Specifically we create Sine \texttt{OsciallatorNode} with frequency 440 HZ, Triangle \texttt{OsciallatorNode} with frequency 10000 HZ, Square \texttt{OsciallatorNode} with frequency 1880 HZ and Sawtooth \texttt{OsciallatorNode} with frequency 22000 HZ. All of these \texttt{OscillatorNode} are then connected to the \texttt{ChannelMergeNode}. The output of the \texttt{ChannelMergeNode} is connected to the \texttt{DynamicCompressorNode} as before. The rest of the Audio Nodes remain the same as previous methods with FFT being captured and hashed through the \emph{onaudioprocess} event handler added by the  \texttt{ScriptProcessorNode}. Figure \ref{fig:ChannelMergeHybrid} shows the exact implementation of the Channel Merge Hybrid method and Figure \ref{fig:GeneratedChannelMergeWave} shows the output of the \texttt{ChannelMergeNode}.

\begin{figure}
    \centering
    \includegraphics[scale=0.5]{WaveForms/ChannelMergeGenerated.png}
    \caption[Generated Channel Merge Wave]{Generated Channel Merge Wave}
    \label{fig:GeneratedChannelMergeWave}
\end{figure}

\subsection{Amplitude Modulation Hybrid Method}
\label{sec: AmplitudeModulation}
\begin{figure}[H]
    \centering
    \includegraphics[width=1.0\columnwidth]{Schematics/AM.pdf}
    \caption[{Amplitude Modulation Hybrid Method}]{Amplitude Modulation Hybrid Method}
    \label{fig:AmplitudeModulationHybrid}
\end{figure}

Amplitude Modulation Hybrid is yet another contribution to the fingerprinting method introduced during this research. The major focus here is also on the signal generation. The rest of the audio nodes remains the same as previous methods where the FFT is being captured and hashed through the \emph{onaudioprocess} event handler added by the  \texttt{ScriptProcessorNode} to generate an audio fingerprint. We introduce two modulating waves: 1) Triangle, 440HZ 2) Square, 18HZ that are connected to their respective \texttt{GainNode}'s. The carrier wave is a Sine wave oscillating at 10000HZ that is connected to its own \texttt{GainNode}. The output of the both Modulating \texttt{GainNode}s are connected to carrier \texttt{GainNode}. This output is then connected to \texttt{DynamicCompressor} and the rest of the stack remains the same as well as the process. Figure \ref{fig:AmplitudeModulationHybrid} shows the exact implementation of the Amplitude Modulation Hybrid method and Figure \ref{fig:GeneratedAmplitudeModulationWave} shows the output of the carrier \texttt{GainNode}.

\begin{figure}
    \centering
    \includegraphics[scale=0.5]{WaveForms/AMGenerated.png}
    \caption[Generated Amplitude Modulation Wave]{Generated Amplitude Modulation Wave}
    \label{fig:GeneratedAmplitudeModulationWave}
\end{figure}

\subsection{Frequency Modulation Hybrid Method}
\label{sec: FrequencyModulation}
\begin{figure}
    \centering
    \includegraphics[scale=0.5]{Schematics/FM.jpg}
    \caption[{Frequency Modulation Hybrid Method}]{Frequency Modulation Hybrid Method}
    \label{fig:FrequencyModualationHybrid}
\end{figure}
Frequency Modulation Hybrid is another add to fingerprinting method introduced during this research. This method is analogous to Amplitude Modulation Hybrid Method discussed to \ref{sec: AmplitudeModulation}. Similar to Amplitude Modulation Hybrid Method we introduce two modulating waves: 1) Triangle, 440HZ 2) Square, 18HZ that are connected to their respective \texttt{GainNode}'s whose gain is set to 60 and 30 respectively. The carrier wave is a Sine wave oscillating at 10000HZ. The output of the both Modulating \texttt{GainNode}'s are connected to carrier frequency. This output is then connected to \texttt{DynamicCompressor}. The rest of the audio nodes remains the same as previous methods where the FFT is being captured and hashed through the \emph{onaudioprocess} event handler added by the  \texttt{ScriptProcessorNode} to generate an audio fingerprint. Figure \ref{fig:FrequencyModualationHybrid} shows the exact implementation of the Frequency Modulation Hybrid method and Figure \ref{fig:GeneratedFrequencyModulationWave} shows the output of the carrier wave.

\begin{figure}
    \centering
    \includegraphics[scale=0.5]{WaveForms/FMGenerated.png}
    \caption[Generated Frequency Modulation Wave]{Generated Frequency Modulation Wave}
    \label{fig:GeneratedFrequencyModulationWave}
\end{figure}

